Double-double radio galaxies from the FIRST survey

The radio structures and optical identifications of a sample of 242 sources classified as double-double radio sources by Proctor (2011) from a morphological study of sources in the FIRST (Faint Images of the Radio Sky at Twenty centimeters) survey (2003 April release, 811,117 entries) have been examined. We have been able to confirm only 23 of these as likely to be double-double radio galaxies (DDRGs), whose structures could be attributed to episodic nuclear activity in their host galaxies. A further 63 require either higher-resolution radio observations or optical identifications to determine whether these are DDRGs. The remaining sources are unlikely to be DDRGs. We have examined the luminosities, sizes and symmetry parameters of the DDRGs and the constraints these place on our understanding of these sources.

==> basi_ddrg <==
\begin{table}
\caption{DDRGs from the FIRST survey}
\label{tab:sample_ddrgs}
{\small
\centering
\begin{tabular}{c c c c c c c c }
\hline




\begin{table}
\caption{ The sample of DDRGs}
\label{tab:ddrgs}
{\small
\centering
\begin{tabular}{l  c  l  rr  c rr rr rr rr l }
\hline
Source       & Opt.& Red- & $l_{in}$& $l_{o}$& Cmp.& R$_{\theta(in)}$ &R$_{\theta(o)}$ & R$_{s(in)}$ &R$_{s(o)}$
& $\Delta_{in}$ & $\Delta_{o}$ & P$_{in}$ & P$_{o}$ & Ref.\\
             & Id. & shift& kpc  & kpc   &     &       &       &        &        & $^\circ$ & $^\circ$ & W/Hz & W/Hz &  \\
    (1)      & (2) &  (3) &  (4) &  (5)  & (6) &  (7)  &  (8)  &  (9)   &  (10)  & (11) & (12)  & (13) & (14)  & (15)  \\
\hline
J0746$+$4526 &  G  &(0.517)& 95   & 630   &N/S  &1.86   &1.35   & 0.79   &0.19    &      &       & 25.41& 26.17 &    \\
J0804$+$5809 &     &       &      &       &W/E  &2.00   &0.99   & 1.43   &0.81    &      &       &      &       &    \\
J0855$+$4204 &  G  &(0.279)& 40   & 516   &N/S  &1.17   &0.86   & 1.34   &0.87    &      &       & 24.64& 25.30 &    \\
J0910$+$0345 &  G  &(0.588)& 34   & 225   &E/W  &2.17   &0.73   & 0.84   &0.99    &      &       & 25.85& 25.66 &    \\
J1039$+$0536 &  G  &0.0908 & 29   & 163   &W/E  &1.25   &0.74   & 1.03   &1.29    &      &       & 24.05& 24.97 &    \\
J1044$+$1442 &  G  &0.1547 &      &       &     &       &       &        &        &      &       & 24.24& 25.23 &    \\
J1103$+$0636 &  G  &(0.449)& 71   & 652   &E/W  &1.28   &0.93   & 1.51   &0.72    &      &       & 24.99& 25.56 &    \\
J1107$+$1216 &  G  &       &      &       &     &       &       &        &        &      &       & 24.35& 24.62 &    \\
J1158$+$2621 &  G  &0.1120 & 143  & 503   &N/S  &1.70   &1.01   & 1.81   &1.31    &      &       & 24.33& 24.80 &    \\
J1208$+$0821 &  G  &(0.600)& 121  & 687   &W/E  &1.07   &1.04   & 0.93   &0.96    &      &       & 24.49& 25.76 &    \\
J1238$+$1602 &  S  &       &      &       &S/N  &1.23   &0.91   & 1.12   &0.79    &      &       &      &       &    \\
J1240$+$2122 &  G  &(0.357)& 67   & 577   &S/N  &2.00   &1.07   & 4.40   &0.72    &      &       & 25.10& 25.42 &    \\
J1326$+$1924 &  G  &0.1762 & 27   & 149   &E/W  &1.20   &1.25   & 1.06   &0.65    &      &       & 23.68& 24.56 &    \\
J1328$+$2752 &  G  &0.0911 & 95   & 355   &N/S  &1.53   &1.61   & 1.85   &0.63    &      &       & 23.76& 24.39 &    \\
J1344$-$0030 &  G  &(0.579)& 86   & 643   &N/S  &1.25   &1.06   & 1.30   &0.35    &      &       & 25.46& 25.60 &    \\
J1407$+$5132 &  G  &(0.324)& 87   & 613   &W/E  &1.40   &0.84   & 1.51   &0.62    &      &       & 24.43& 26.15 &    \\
J1500$+$1542 &  G  &(0.456)& 128  & 485   &S/N  &1.54   &0.76   & 1.68   &1.27    &      &       & 24.93& 24.92 &    \\
J1521$+$5214 &  G  &(0.537)& 64.  & 391   &S/N  &1.50   &0.74   & 2.09   &0.81    &      &       & 24.99& 25.28 &    \\              
J1538$-$0242 &  G  &(0.575)& 59   & 534   &N/S  &1.16   &0.93   & 0.73   &1.24    &      &       & 25.05& 26.30 &    \\
J1545$+$5047 &  G  &0.4309 & 66   & 483   &E/W  &1.12   &0.84   & 0.67   &1.23    &      &       & 24.95& 25.69 &    \\
J1605$+$0711 &  G  &(0.268)&799   & 576   &S/N  &1.30   &1.06   & 0.54   &0.69    &      &       & 25.05& 25.38 &    \\
J1627$+$2906 &  G  &(0.722)& 74   & 702   &N/S  &2.20   &0.98   & 0.80   &1.46    &      &       & 25.40& 26.30 &    \\
J1649$+$4133 &  S  &       &      &       &E/W  &1.25   &0.94   & 1.38   &1.66    &      &       &      &       &    \\                 
J1705$+$3940 &  G  &(0.701)& 130  & 528   &S/N  &1.70   &0.96   & 2.52   &1.27    &      &       & 25.84& 26.07 &    \\
J1706$+$4340 &     &       &      &       &S/N  &1.24   &0.98   & 8.67   &0.59    &      &       &              &    \\        
\hline
\end{tabular}


